A multi-agent model for growing spiking neural networks

Artificial Intelligence has looked into biological systems as a source of inspiration. Although there are many aspects of the brain yet to be discovered, neuroscience has found evidence that the connections between neurons continuously grow and reshape as a part of the learning process. This differs from the design of Artificial Neural Networks, that achieve learning by evolving the weights in the synapses between them and their topology stays unaltered through time. This project has explored rules for growing the connections between the neurons in Spiking Neural Networks as a learning mechanism. These rules have been implemented on a multi-agent system for creating simple logic functions, that establish a base for building up more complex systems and architectures. Results in a simulation environment showed that for a given set of parameters it is possible to reach topologies that reproduce the tested functions. This project also opens the door to the usage of techniques like genetic algorithms for obtaining the best suited values for the model parameters, and hence creating neural networks that can adapt to different functions.

==> reviews/firing_models.tex <==


\paragraph{Izhikevich model:\\}


Classic models of the biological neuron establish that the output is the result of integrating through time the received information, and neurons get excited based on the average values of incoming pulses. However, more recent approaches assume that neurons work as temporal detectors that react based on the temporal coincidence of input spikes i.e. there is a correlation between the timing of the input spikes and the excitation of the neuron \citep{konig1996integrator}. In terms of computation, this change lead to a remarkable increase in the encoding alternatives for a given set of neurons, as the spiking time turns to be a new dimension. Moreover, the reaction time of a network is considerably faster, as a spike is enough for provoking a change in the output.

\begin{displayquote}
\textit{This concept [neurons operating as coincidence detectors] assumes that temporal correlations among spatially separate neurons are crucial for processing as part of the information is coded in the temporal structure of activity patterns} \citep{konig1996integrator}.
\end{displayquote}


Neuromorphic engineering has been exploring the behaviour of the biological neurons and several models for reproducing them have been proposed. They primarily look for a trade off between computational costs and their fidelity to the actual behaviour of biological neurons. In this search, the model proposed by \citep{izhikevich2003simple} has proved to resemble real neurons while keeping a low computational cost. The model is a reduction of the Hodgin-Huxley model, and is summarized by the system of 2 differential equations shown in eq. \ref{eq:izhikevich},

\begin{empheq}[left=\empheqlbrace]{align}
    \label{eq:izhikevich}
    &v' = 0.04v^2 + 5v + 140 - u + I \nonumber \\
    && \\
    &u' = a(bv - u) \nonumber
\end{empheq}

where \textit{v} represents the membrane potential of the neuron, and \textit{u} its recovery variable. Eq. \ref{eq:izhikevich} is completed with the resetting rule shown in eq. \ref{eq:izhikevich_reset}, applied when \textit{v} reaches the threshold membrane potential.

\begin{empheq}[left=\empheqlbrace]{align}
    \label{eq:izhikevich_reset}
    & v  \longleftarrow c \nonumber \\
    &u \longleftarrow u + d
\end{empheq}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/coincidence_detector/izhikevich.png}
    \caption{Shape of the neuron model proposed by Izhikevich for SNNs \citep{izhikevich2003simple}. Figure obtained at the website of the \textit{University of Sidney} \footnote{\url{http://www.physics.usyd.edu.au/teach_res/mp/ns/doc/nsIzhikevich3.htm}}.}
    \label{fig:my_label}
\end{figure}



\paragraph{Leaky Integrate and Fire:\\}


\paragraph{Galves-Löcherbach model:\\}

This model introduces a stochastic process for deciding when a neuron triggers. The probability of triggering increases with the membrane potential of the neuron


\paragraph{Linear-nonlinear-Poisson cascade model:\\}

